Divide & Bind Your Attention for Improved Generative Semantic Nursing

Emerging large-scale text-to-image generative models, e.g., Stable Diffusion (SD), have exhibited overwhelming results with high fidelity. Despite the magnificent progress, current state-of-the-art models still struggle to generate images fully adhering to the input prompt. Prior work, Attend & Excite, has introduced the concept of Generative Semantic Nursing (GSN), aiming to optimize cross-attention during inference time to better incorporate the semantics. It demonstrates promising results in generating simple prompts, e.g., "a cat and a dog". However, its efficacy declines when dealing with more complex prompts, and it does not explicitly address the problem of improper attribute binding. To address the challenges posed by complex prompts or scenarios involving multiple entities and to achieve improved attribute binding, we propose Divide & Bind. We introduce two novel loss objectives for GSN: a novel attendance loss and a binding loss. Our approach stands out in its ability to faithfully synthesize desired objects with improved attribute alignment from complex prompts and exhibits superior performance across multiple evaluation benchmarks.

==> fig/attention_tex.tex <==

\begin{figure*}[t]
\begin{centering}
\setlength{\tabcolsep}{0.0em}
\renewcommand{\arraystretch}{0}
\par\end{centering}
\begin{centering}
%\vspace{-2em}
\hfill{}%
	\begin{tabular}{
    m{1.5em}<{\centering} %@{\hspace{1em}}
    m{0.15\linewidth}<{\centering} @{\hspace{-1em}}
    m{0.15\linewidth}<{\centering}  @{}%@{\hspace{-5em}}
    m{0.15\linewidth}<{\centering} @{}
    m{0.15\linewidth}<{\centering}
    }
    &
    \multicolumn{4}{c}{\hspace{-0.02\linewidth}\myquote{A \textblue{dog} and a \textblue{turtle} on the street, snowy scene}} 
    
    \tabularnewline
    &
    $x_0$
    & \hspace{3em}$\hat{x_0}^{(t)}$\hspace{-1em}
    & %{\hspace{4em} } %{\footnotesize{}}
    \hspace{2em}dog
    & %{\footnotesize{}} {\hspace{4em} }
     \hspace{-1em}turtle
	%\vspace{0.02cm} 
    %% Stable Diffsuion
    \tabularnewline
    \multirow{1}{*}{\rotatebox{90}{
        \hspace{2.2em}
        \begin{tabular}{c}
        \small Stable\\ \small Diffusion 
        \end{tabular}
        \hspace{-2.2em}
    }} 
    &
    \includegraphics[ height=0.09\textheight]{fig/attn_gif_v2/a_dog_and_a_turtle_on_the_street,snowy_driving_sce_seed8099.jpg}
    &
    \multicolumn{3}{c}{\begin{tabular}{c}\animategraphics[autoplay,loop,height=0.09\textheight]{3}{fig/attn_gif_v2/SD/}{0}{41}\end{tabular}} 
    
	 %% Attend and Excite
  \tabularnewline
  \multirow{1}{*}{\rotatebox{90}{
        \hspace{2.4em}
        \begin{tabular}{c<{\centering}}
        \small
        Attend \& \\ \small Excite
        \end{tabular}
        \hspace{-2.4em}
    }} 
    &
    \includegraphics[height=0.09\textheight]{fig/attn_gif_v2/a_dog_and_a_turtle_on_the_street,snowy_driving_sce_seed8099_attend_max_stepInit50_0.jpg}
    &
    \multicolumn{3}{c}{\begin{tabular}{c}\animategraphics[autoplay,loop,height=0.09\textheight]{3}{fig/attn_gif_v2/AE/}{0}{41}\end{tabular}} 
	 \tabularnewline
  %% Ours
    \multirow{1}{*}{\rotatebox{90}{
        \hspace{3.5em}
        \begin{tabular}{c}
        \small
        \textbf{{\ours}}\\
        \small (Ours) 
        \end{tabular}
        \hspace{-3.5em}
    }} 
    &
    \includegraphics[height=0.09\textheight]{fig/attn_gif_v2/a_dog_and_a_turtle_on_the_street,snowy_driving_sce_seed8099_attend_tv_stepInit50_0.jpg}
    &
    \multicolumn{3}{c}{\begin{tabular}{c}\animategraphics[autoplay,loop,height=0.09\textheight]{3}{fig/attn_gif_v2/TV/}{0}{41}\end{tabular}} 

    \tabularnewline
	\end{tabular}
\hfill{}
\par\end{centering}
\caption{
Cross-attention visualization in different timesteps for each object token and predicted clean image $\hat{x_0}^{(t)}$.
Note that this is GIF, video version can be found on the \href{https://sites.google.com/view/divide-and-bind}{project page}.
} 
\label{fig:attention_vis}
%\vspace{-1em}
\end{figure*}



==> fig/visual_JSD.tex <==
% %%%%%%  Teaser Comparison %%%%%%

\begin{figure*}[t]
\centering
\includegraphics[width=0.7\linewidth]{fig/dummy_pic_bear.jpg}
\caption{\textbf{Visual} visual comparison with and without JSD
}
\label{fig:teaser}
%\vspace{-1.0em}
\end{figure*}

% \begin{figure}[t]
%     \begin{centering}
%     \setlength{\tabcolsep}{0.0em}
%     \renewcommand{\arraystretch}{0}
%     \par\end{centering}
%     \begin{centering}
%     \vspace{-0.5em}
%     \hfill{}%
%     %\vspace{1ex}
% 	%height=0.105\textwidth
% 	\begin{tabular}{@{}c@{}c}
%         \centering
% 		\small Content &  \small Style   \tabularnewline
% 		\includegraphics[width=0.45\linewidth]{figs/masking_ablation_2x2/weimar_000069_000019_leftImg8bit.jpg} &
% 		{\hspace{0.5em}} \includegraphics[width=0.45\linewidth]{figs/masking_ablation_2x2/darmstadt_000004_000019_leftImg8bit.jpg} \tabularnewline
% 	     \small W/o masking & \small W/- masking (Ours)  \tabularnewline
% 		\includegraphics[width=0.45\linewidth]{figs/masking_ablation_2x2/darmstadt_000004_000019_without_mask.jpg} & {\hspace{0.5em}}
% 		\includegraphics[width=0.45\linewidth]{figs/masking_ablation_2x2/darmstadt_000004_000019_with_mask.jpg} 
% 		\tabularnewline
  
% % 		\includegraphics[width=0.241\textwidth]{figs/masking_ablation/2_content_9.jpg}  &
% % 	{\footnotesize{}}	\includegraphics[width=0.241\textwidth]{figs/masking_ablation/2_style_17.jpg} & {\footnotesize{}}
% % 		\includegraphics[width=0.241\textwidth]{figs/masking_ablation/2_masking_swap_9_17.jpg} & {\footnotesize{}}
% % 		\includegraphics[width=0.241\textwidth]{figs/masking_ablation/2_no_masking_swap_9_17.jpg} \tabularnewline
% 		\end{tabular}
% \hfill{}
% \par\end{centering}
% %\vspace{-0.5em}
% \caption{Style mixing effect enabled by random noise masking (best view in color). Despite the good reconstruction quality, the encoder trained without masking cannot change the style of the given $\mathrm{Content}$ image. In contrast, the encoder trained with masking can modify it using the style from the given $\mathrm{Style}$ image.}
% \label{fig:masking-ablation}
% \vspace{-0.7em}
% \end{figure}
